Peta-electron volt gamma-ray emission from the Crab Nebula

The Crab pulsar and the surrounding nebula powered by the pulsar's rotational energy through the formation and termination of a relativistic electron-positron wind is a bright source of gamma-rays carrying crucial information about this complex conglomerate. We report the detection of $\gamma$-rays with a spectrum showing gradual steepening over three energy decades, from $5\times 10^{-4}$ to $1.1$ petaelectronvolt (PeV). The ultra-high-energy photons exhibit the presence of a PeV electron accelerator (a pevatron) with an acceleration rate exceeding 15% of the absolute theoretical limit. Assuming that unpulsed $\gamma$-rays are produced at the termination of the pulsar's wind, we constrain the pevatron's size, between $0.025$ and $0.1$ pc, and the magnetic field $\approx 110 \mu$G. The production rate of PeV electrons, $2.5 \times 10^{36}$ erg $\rm s^{-1}$, constitutes 0.5% of the pulsar's spin-down luminosity, although we do not exclude a non-negligible contribution of PeV protons to the production of the highest energy $\gamma$-rays.

==> author20210531.tex <==
%%updated in 2021-05-31 by Chen Songzhan
%%please send email to chensz@ihep.ac.cn for any problem
\author{
\noindent
Zhen Cao$^{1,2,3}$,
F. Aharonian$^{4,5}$,
Q. An$^{6,7}$,
Axikegu$^{8}$,
L.X. Bai$^{9}$,
Y.X. Bai$^{1,3}$,
Y.W. Bao$^{10}$,
D. Bastieri$^{11}$,
X.J. Bi$^{1,2,3}$,
Y.J. Bi$^{1,3}$,
H. Cai$^{12}$,
J.T. Cai$^{11}$,
Zhe Cao$^{6,7}$,
J. Chang$^{13}$,
J.F. Chang$^{1,3,6}$,
B.M. Chen$^{14}$,
E.S. Chen$^{1,2,3}$,
J. Chen$^{9}$,
Liang Chen$^{1,2,3}$,
Liang Chen$^{15}$,
Long Chen$^{8}$,
M.J. Chen$^{1,3}$,
M.L. Chen$^{1,3,6}$,
Q.H. Chen$^{8}$,
S.H. Chen$^{1,2,3}$,
S.Z. Chen$^{1,3}$,
T.L. Chen$^{16}$,
X.L. Chen$^{1,2,3}$,
Y. Chen$^{10}$,
N. Cheng$^{1,3}$,
Y.D. Cheng$^{1,3}$,
S.W. Cui$^{14}$,
X.H. Cui$^{17}$,
Y.D. Cui$^{18}$,
B. D'Ettorre Piazzoli$^{19}$,
B.Z. Dai$^{20}$,
H.L. Dai$^{1,3,6}$,
Z.G. Dai$^{7}$,
Danzengluobu$^{16}$,
D. della Volpe$^{21}$,
X.J. Dong$^{1,3}$,
K.K. Duan$^{13}$,
J.H. Fan$^{11}$,
Y.Z. Fan$^{13}$,
Z.X. Fan$^{1,3}$,
J. Fang$^{20}$,
K. Fang$^{1,3}$,
C.F. Feng$^{22}$,
L. Feng$^{13}$,
S.H. Feng$^{1,3}$,
Y.L. Feng$^{13}$,
B. Gao$^{1,3}$,
C.D. Gao$^{22}$,
L.Q. Gao$^{1,2,3}$,
Q. Gao$^{16}$,
W. Gao$^{22}$,
M.M. Ge$^{20}$,
L.S. Geng$^{1,3}$,
G.H. Gong$^{23}$,
Q.B. Gou$^{1,3}$,
M.H. Gu$^{1,3,6}$,
F.L. Guo$^{15}$,
J.G. Guo$^{1,2,3}$,
X.L. Guo$^{8}$,
Y.Q. Guo$^{1,3}$,
Y.Y. Guo$^{1,2,3,13}$,
Y.A. Han$^{24}$,
H.H. He$^{1,2,3}$,
H.N. He$^{13}$,
J.C. He$^{1,2,3}$,
S.L. He$^{11}$,
X.B. He$^{18}$,
Y. He$^{8}$,
M. Heller$^{21}$,
Y.K. Hor$^{18}$,
C. Hou$^{1,3}$,
X. Hou$^{25}$,
H.B. Hu$^{1,2,3}$,
S. Hu$^{9}$,
S.C. Hu$^{1,2,3}$,
X.J. Hu$^{23}$,
D.H. Huang$^{8}$,
Q.L. Huang$^{1,3}$,
W.H. Huang$^{22}$,
X.T. Huang$^{22}$,
X.Y. Huang$^{13}$,
Z.C. Huang$^{8}$,
F. Ji$^{1,3}$,
X.L. Ji$^{1,3,6}$,
H.Y. Jia$^{8}$,
K. Jiang$^{6,7}$,
Z.J. Jiang$^{20}$,
C. Jin$^{1,2,3}$,
T. Ke$^{1,3}$,
D. Kuleshov$^{26}$,
K. Levochkin$^{26}$,
B.B. Li$^{14}$,
Cheng Li$^{6,7}$,
Cong Li$^{1,3}$,
F. Li$^{1,3,6}$,
H.B. Li$^{1,3}$,
H.C. Li$^{1,3}$,
H.Y. Li$^{7,13}$,
Jie Li$^{1,3,6}$,
Jian Li$^{7}$,
K. Li$^{1,3}$,
W.L. Li$^{22}$,
X.R. Li$^{1,3}$,
Xin Li$^{6,7}$,
Xin Li$^{8}$,
Y. Li$^{9}$,
Y.Z. Li$^{1,2,3}$,
Zhe Li$^{1,3}$,
Zhuo Li$^{27}$,
E.W. Liang$^{28}$,
Y.F. Liang$^{28}$,
S.J. Lin$^{18}$,
B. Liu$^{7}$,
C. Liu$^{1,3}$,
D. Liu$^{22}$,
H. Liu$^{8}$,
H.D. Liu$^{24}$,
J. Liu$^{1,3}$,
J.L. Liu$^{29}$,
J.S. Liu$^{18}$,
J.Y. Liu$^{1,3}$,
M.Y. Liu$^{16}$,
R.Y. Liu$^{10}$,
S.M. Liu$^{8}$,
W. Liu$^{1,3}$,
Y. Liu$^{11}$,
Y.N. Liu$^{23}$,
Z.X. Liu$^{9}$,
W.J. Long$^{8}$,
R. Lu$^{20}$,
H.K. Lv$^{1,3}$,
B.Q. Ma$^{27}$,
L.L. Ma$^{1,3}$,
X.H. Ma$^{1,3}$,
J.R. Mao$^{25}$,
A. Masood$^{8}$,
Z. Min$^{1,3}$,
W. Mitthumsiri$^{30}$,
T. Montaruli$^{21}$,
Y.C. Nan$^{22}$,
B.Y. Pang$^{8}$,
P. Pattarakijwanich$^{30}$,
Z.Y. Pei$^{11}$,
M.Y. Qi$^{1,3}$,
Y.Q. Qi$^{14}$,
B.Q. Qiao$^{1,3}$,
J.J. Qin$^{7}$,
D. Ruffolo$^{30}$,
V. Rulev$^{26}$,
A. S\'aiz$^{30}$,
L. Shao$^{14}$,
O. Shchegolev$^{26,31}$,
X.D. Sheng$^{1,3}$,
J.Y. Shi$^{1,3}$,
H.C. Song$^{27}$,
Yu.V. Stenkin$^{26,31}$,
V. Stepanov$^{26}$,
Y. Su$^{13}$,
Q.N. Sun$^{8}$,
X.N. Sun$^{28}$,
Z.B. Sun$^{32}$,
P.H.T. Tam$^{18}$,
Z.B. Tang$^{6,7}$,
W.W. Tian$^{2,17}$,
B.D. Wang$^{1,3}$,
C. Wang$^{32}$,
H. Wang$^{8}$,
H.G. Wang$^{11}$,
J.C. Wang$^{25}$,
J.S. Wang$^{29}$,
L.P. Wang$^{22}$,
L.Y. Wang$^{1,3}$,
R.N. Wang$^{8}$,
W. Wang$^{18}$,
W. Wang$^{12}$,
X.G. Wang$^{28}$,
X.J. Wang$^{1,3}$,
X.Y. Wang$^{10}$,
Y. Wang$^{8}$,
Y.D. Wang$^{1,3}$,
Y.J. Wang$^{1,3}$,
Y.P. Wang$^{1,2,3}$,
Z.H. Wang$^{9}$,
Z.X. Wang$^{20}$,
Zhen Wang$^{29}$,
Zheng Wang$^{1,3,6}$,
D.M. Wei$^{13}$,
J.J. Wei$^{13}$,
Y.J. Wei$^{1,2,3}$,
T. Wen$^{20}$,
C.Y. Wu$^{1,3}$,
H.R. Wu$^{1,3}$,
S. Wu$^{1,3}$,
W.X. Wu$^{8}$,
X.F. Wu$^{13}$,
S.Q. Xi$^{1,3}$,
J. Xia$^{7,13}$,
J.J. Xia$^{8}$,
G.M. Xiang$^{2,15}$,
D.X. Xiao$^{16}$,
G. Xiao$^{1,3}$,
H.B. Xiao$^{11}$,
G.G. Xin$^{12}$,
Y.L. Xin$^{8}$,
Y. Xing$^{15}$,
D.L. Xu$^{29}$,
R.X. Xu$^{27}$,
L. Xue$^{22}$,
D.H. Yan$^{25}$,
J.Z. Yan$^{13}$,
C.W. Yang$^{9}$,
F.F. Yang$^{1,3,6}$,
J.Y. Yang$^{18}$,
L.L. Yang$^{18}$,
M.J. Yang$^{1,3}$,
R.Z. Yang$^{7}$,
S.B. Yang$^{20}$,
Y.H. Yao$^{9}$,
Z.G. Yao$^{1,3}$,
Y.M. Ye$^{23}$,
L.Q. Yin$^{1,3}$,
N. Yin$^{22}$,
X.H. You$^{1,3}$,
Z.Y. You$^{1,2,3}$,
Y.H. Yu$^{22}$,
Q. Yuan$^{13}$,
H.D. Zeng$^{13}$,
T.X. Zeng$^{1,3,6}$,
W. Zeng$^{20}$,
Z.K. Zeng$^{1,2,3}$,
M. Zha$^{1,3}$,
X.X. Zhai$^{1,3}$,
B.B. Zhang$^{10}$,
H.M. Zhang$^{10}$,
H.Y. Zhang$^{22}$,
J.L. Zhang$^{17}$,
J.W. Zhang$^{9}$,
L.X. Zhang$^{11}$,
Li Zhang$^{20}$,
Lu Zhang$^{14}$,
P.F. Zhang$^{20}$,
P.P. Zhang$^{14}$,
R. Zhang$^{7,13}$,
S.R. Zhang$^{14}$,
S.S. Zhang$^{1,3}$,
X. Zhang$^{10}$,
X.P. Zhang$^{1,3}$,
Y.F. Zhang$^{8}$,
Y.L. Zhang$^{1,3}$,
Yi Zhang$^{1,13}$,
Yong Zhang$^{1,3}$,
B. Zhao$^{8}$,
J. Zhao$^{1,3}$,
L. Zhao$^{6,7}$,
L.Z. Zhao$^{14}$,
S.P. Zhao$^{13,22}$,
F. Zheng$^{32}$,
Y. Zheng$^{8}$,
B. Zhou$^{1,3}$,
H. Zhou$^{29}$,
J.N. Zhou$^{15}$,
P. Zhou$^{10}$,
R. Zhou$^{9}$,
X.X. Zhou$^{8}$,
C.G. Zhu$^{22}$,
F.R. Zhu$^{8}$,
H. Zhu$^{17}$,
K.J. Zhu$^{1,2,3,6}$,
X. Zuo$^{1,3}$
(The LHAASO Collaboration)
}\\
\footnotesize{
\noindent
$^{1}$ Key Laboratory of Particle Astrophyics \& Experimental Physics Division \& Computing Center, Institute of High Energy Physics, Chinese Academy of Sciences, 100049 Beijing, China\\
$^{2}$ University of Chinese Academy of Sciences, 100049 Beijing, China\\
$^{3}$ TIANFU Cosmic Ray Research Center, Chengdu, Sichuan,  China\\
$^{4}$ Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, 2 Dublin, Ireland \\
$^{5}$ Max-Planck-Institut for Nuclear Physics, P.O. Box 103980, 69029  Heidelberg, Germany\\
$^{6}$ State Key Laboratory of Particle Detection and Electronics, China\\
$^{7}$ University of Science and Technology of China, 230026 Hefei, Anhui, China\\
$^{8}$ School of Physical Science and Technology \&  School of Information Science and Technology, Southwest Jiaotong University, 610031 Chengdu, Sichuan, China\\
$^{9}$ College of Physics, Sichuan University, 610065 Chengdu, Sichuan, China\\
$^{10}$ School of Astronomy and Space Science, Nanjing University, 210023 Nanjing, Jiangsu, China\\
$^{11}$ Center for Astrophysics, Guangzhou University, 510006 Guangzhou, Guangdong, China\\
$^{12}$ School of Physics and Technology, Wuhan University, 430072 Wuhan, Hubei, China\\
$^{13}$ Key Laboratory of Dark Matter and Space Astronomy, Purple Mountain Observatory, Chinese Academy of Sciences, 210023 Nanjing, Jiangsu, China\\
$^{14}$ Hebei Normal University, 050024 Shijiazhuang, Hebei, China\\
$^{15}$ Key Laboratory for Research in Galaxies and Cosmology, Shanghai Astronomical Observatory, Chinese Academy of Sciences, 200030 Shanghai, China\\
$^{16}$ Key Laboratory of Cosmic Rays (Tibet University), Ministry of Education, 850000 Lhasa, Tibet, China\\
$^{17}$ National Astronomical Observatories, Chinese Academy of Sciences, 100101 Beijing, China\\
$^{18}$ School of Physics and Astronomy \& School of Physics (Guangzhou), Sun Yat-sen University, 519000 Zhuhai, Guangdong, China\\
$^{19}$ Dipartimento di Fisica dell'Universit\`a di Napoli \``Federico II'', Complesso Universitario di Monte Sant'Angelo, via Cinthia, 80126 Napoli, Italy. \\
$^{20}$ School of Physics and Astronomy, Yunnan University, 650091 Kunming, Yunnan, China\\
$^{21}$ D'epartement de Physique Nucl'eaire et Corpusculaire, Facult'e de Sciences, Universit'e de Gen\`eve, 24 Quai Ernest Ansermet, 1211 Geneva, Switzerland\\
$^{22}$ Institute of Frontier and Interdisciplinary Science, Shandong University, 266237 Qingdao, Shandong, China\\
$^{23}$ Department of Engineering Physics, Tsinghua University, 100084 Beijing, China\\
$^{24}$ School of Physics and Microelectronics, Zhengzhou University, 450001 Zhengzhou, Henan, China\\
$^{25}$ Yunnan Observatories, Chinese Academy of Sciences, 650216 Kunming, Yunnan, China\\
$^{26}$ Institute for Nuclear Research of Russian Academy of Sciences, 117312 Moscow, Russia\\
$^{27}$ School of Physics, Peking University, 100871 Beijing, China\\
$^{28}$ School of Physical Science and Technology, Guangxi University, 530004 Nanning, Guangxi, China\\
$^{29}$ Tsung-Dao Lee Institute \& School of Physics and Astronomy, Shanghai Jiao Tong University, 200240 Shanghai, China\\
$^{30}$ Department of Physics, Faculty of Science, Mahidol University, 10400 Bangkok, Thailand\\
$^{31}$ Moscow Institute of Physics and Technology, 141700 Moscow, Russia\\
$^{32}$ National Space Science Center, Chinese Academy of Sciences, 100190 Beijing, China\\
}


